A rational QZ method

We propose a rational QZ method for the solution of the dense, unsymmetric generalized eigenvalue problem. This generalization of the classical QZ method operates implicitly on a Hessenberg, Hessenberg pencil instead of on a Hessenberg, triangular pencil. Whereas the QZ method performs nested subspace iteration driven by a polynomial, the rational QZ method allows for nested subspace iteration driven by a rational function, this creates the additional freedom of selecting poles. In this article we study Hessenberg, Hessenberg pencils, link them to rational Krylov subspaces, propose a direct reduction method to such a pencil, and introduce the implicit rational QZ step. The link with rational Krylov subspaces allows us to prove essential uniqueness (implicit Q theorem) of the rational QZ iterates as well as convergence of the proposed method. In the proofs, we operate directly on the pencil instead of rephrasing it all in terms of a single matrix. Numerical experiments are included to illustrate competitiveness in terms of speed and accuracy with the classical approach. Two other types of experiments exemplify new possibilities. First we illustrate that good pole selection can be used to deflate the original problem during the reduction phase, and second we use the rational QZ method to implicitly filter a rational Krylov subspace in an iterative method.

==> sections/07_tightly_packed_shifts/tightly_packed_shifts.tex <==
\section{Tightly packed shifts.}
\label{sec:tightly_packed}

The single shift RQZ algorithm of section~\ref{sec:rqz} is prone to two shortcomings
that prohibit to fully exploit the efficiency of modern day computer architectures.
The first is a lack of parallelism.
All operations need to be performed sequentially.
This is a common weakness that none of the algorithms of QR-type have overcome.
Secondly, cache use for larger problems is suboptimal.
This issue can be addressed by increasing the multiplicity of the implicit step
such that multiple computations can be performed on the part of the matrix that is
in memory.
There are two ways to achieve the higher multiplicity.
The first one is a multishift step that generalizes similar results of QR and QZ algorithms \cite{XXXXX}.
However, multishift algorithms tend to suffer from \emph{shift blurring} \cite{Kagstrom2007}.
This is the effect that the shifts in a multishift algorithm can become very imprecise.
They sometimes loose close to all digits of precision throughout an iteration which
slows down the convergence. 
This can already happen for small to moderate multiplicities.
A second possibility is to tightly pack the single shifts together by introducing 
them one after the other in the pair and by chasing them down in one batch.
This effectively solves the problem of shift blurring.

In this section we formulate an RQZ iteration with $m$ tightly packed shifts.
This is a minor generalization of the algorithm of section~\ref{sec:rqz} and
the method consists out of the same three phases.

The tightly packed RQZ method starts from an $n{\times}n$ proper Hessenberg pair $(A,B)$
and chases one batch of $m$ shifts via the following procedure:

\paragraph{Initialization.}
First, $m$ shifts $\varrho_1, \hdots, \varrho_m$ are computed.
Typically the eigenvalues of the lower $m{\times}m$ block of $(A,B)$ are used as shifts.
These can be efficiently computed with the single shift RQZ method.
Next, these shifts are introduced in the Hessenberg pair.
This is accomplished via a procedure similar to the direction reduction algorithm of section~\ref{sec:dirred}.
We start by introducing shift $\varrho_m$ as the first pole. 
Afterwards $\varrho_m$ is swapped $m{-}1$ times to place it at the position of the $m$th pole.
The second shift $\varrho_{m-1}$ is now introduced and swapped $m{-}2$ times to the position of pole $m{-}1$.
This procedure is repeated until all $m$ shifts have been introduced in order.

\paragraph{Chase.}
In order to chase the block of $m$ shifts one row down and one column to the right, 
the adjacent pole on the right side of the block needs to be swapped with $\varrho_m$, $\varrho_{m-1}$,
up to $\varrho_1$ individually.

This adds up to a total of $m$ elementary equivalence transformations which can be accumulated to update
the necessary parts of the matrices in a more cache efficient manner.
The first step in the chasing algorithm of the RQZ method with $m=4$ tightly packed shifts is
illustrated in figure~\ref{fig:tightlypackedswap}.

\begin{figure}[htp]
\label{fig:tightlypackedswap}
\centering
\input{../fig/fig_multishift_2.tikz}
\caption{First swap in the RQZ method with $m=4$ tightly packed shifts.
The Hessenberg pair is drawn in light gray.
The magnified portions show the $4$ shifts $\odot{/}\oslash$ right after the initialization phase
and indicates how they can all be swapped with the next pole $\oplus{/}\ominus$ by four elementary swaps.
These transformation are computed based on the shaded regions in the magnified area.
The dotted sections in the matrix pair are the rows and columns that can be updated efficiently after the swap.}
\end{figure}

\paragraph{Finalization.}
The finalization phase commences when the $m$ shifts occupy the last subdiagonal positions in the Hessenberg pair.
This procedure is a completely analogous to the initialization phase.
First, $m$ new poles $\hat{\xi}_{n-m}, \hdots, \hat{\xi}_{n-1}$ are computed.
Next, they are brought in the Hessenberg pair and placed at the $m$ last subdiagonal 
positions via the procedure of changing the pole $\xi_{n-1}$ and swapping it upwards.
This simultaneously introduces the new poles and extracts the shifts from the Hessenberg pair.
This concludes one RQZ step with tightly packed shifts.

Deflation in a tightly packed RQZ iteration can be monitored according to the exact same criteria as in the 
single shift case since the pair remains in Hessenberg form throughout the iteration.

\subsection{Numerical experiment.}
\label{subsec:example3}
We test the tightly packed RQZ method on randomly generated matrix pairs, 
similar to the experiment in section~\ref{subsec:example2}.
To this end, three problems of sizes $500$, $1000$, and $2000$ are generated
and reduced to Hessenberg pairs with poles at infinity.
This again requires no additional computational work compared to the QZ method,
and allows for a fair comparison.
Next, the tightly packed RQZ method is applied with element-wise deflation criterion
and shift batches of sizes $m = 2, 4, 8, 16, 32$.
The shifts are allows computed as the eigenvalues of the trailing $m{\times}m$ block
with the single shift RQZ method.
The poles are selected following the same four criteria as used in section~\ref{subsec:example2}:
poles at infinity, at zero, Wilkinson poles as the eigenvalues of the leading $m{\times}m$ block,
and randomly generated poles.

Figure~\ref{fig:numexp3_1} displays the relative backward error on the left and 
the average number of iterations per eigenvalue on the right,
both are shown in function of batch size $m$.
We observe that the backward error grows both with problem size and batch size,
but remains small at all times.
The increasing backward error is due to the increase in total operations.
The iterations per eigenvalue decrease with $m$, the slope of the expected
speedup matches the experimental results.
This indicates that no shift blurring or other effects slow down the convergence
of the tightly packed RQZ method.

% COLORS
\definecolor{c500}{RGB}{180, 180, 180}
\definecolor{c1000}{RGB}{90, 90, 90}
\definecolor{c2000}{RGB}{0, 0, 0}

\begin{figure}[htp]
\centering
\input{../fig/numexp3/fig_numexp3_1.tikz}
\caption{(I.) Relative backward error in function of batch size $m$ for the four different pole strategies 
and three different problems of sizes 500 (\ref{line:ne3_c500}), 1000 (\ref{line:ne3_c1000}), 
and 2000 (\ref{line:ne3_c2000}). The error on $A$ is displayed with a dashed line, for $B$ with a full line. 
The lines without markers show the error on the reduction to Hessenberg form. (II.) Average number of iterations
per eigenvalue in function of batch size $m$ for the four pole strategies and three problems. The dotted line indicates
the expected speedup.}
\label{fig:numexp3_1}
\end{figure}

Figure~\ref{fig:numexp3_2} displays the performance of the pole strategies relative to the
choice of poles at infinity in function of batch size (left) and of problem size (right).
The results are comparable with the observations of the experiment in section~\ref{subsec:example2}.
The Wilkinson poles are about $5\%$ more efficient than poles at infinity.
Random poles perform worst in terms of problem size. 
The performance of the poles at zero deteriorates with increasing batch size.
As the problem is initialized with all its poles at infinity, we expect worse performance
for the poles at zero. The reason why this effect is magnified for increasing batch sizes is
unclear.

\begin{figure}[htp]
\centering
\input{../fig/numexp3/fig_numexp3_2.tikz}
\caption{(I.) Performance of the pole strategies relative to the QZ method (infinity) in function of batch size $m$, 
averaged over three problem sizes; and (II.) in function of problem size $n$, averaged over the five batch sizes.}
\label{fig:numexp3_2}
\end{figure}

We conclude from this experiment that the tightly packed variant of the RQZ method has the
same advantages as the single shift version. 
A good choice of poles can speedup the convergence of the method.


==> sections/xx_multishift.tex/multishift.tex <==
\section{Implicitly multishifted rational QZ step}
\label{ssec:multishift}

%In this section we will extend the results of the previous section to arrive at a
%multishift algorithm. 
\Cref{alg:rqz1} can be readily extended to accommodate an implicit RQZ step of higher degree.
The multishift algorithm proceeds similar to \cref{alg:rqz1} in the sense that it consists out of the same three phases: the introduction of a multishift block in $(A,B)$, swapping the block along the subdiagonal, and finalizing the step by introducing new poles. 
As some more machinery is needed in the development of these steps, we present each phase
more elaborately.

For theoretical simplicity, even though not required in practice, we assume $B$
nonsingular. XXXXXXXXXXXXXXXXXXXXXXXXXXx Voor pencisl van de reductie OK, anders? XXXXXXX
Moeten we daar nog iets over zeggen??? XXXXXXXXXX




\subsection{Introducing the shifts}
Given a proper Hessenberg pair $(A,B)$ with poles $\Xi = \lbrace \xi_1$, $\hdots$, $\xi_{n-1}\rbrace$ and $m < n$ shifts $\Rho = \lbrace \varrho_1, \hdots \varrho_m \rbrace$, $\Rho \cap \Xi_{1:m} = \varnothing$. 
The $m$ shifts can be introduced simultaneously in the leading corner of $(A,B)$. To this end, consider the vector:
\begin{equation}
\label{eq:vec_multishift}
\bm{x} = \gamma \LinOp{\mu_m}{\nu_m} \LinOpInv{\alpha_m}{\beta_m} \hdots \LinOp{\mu_1}{\nu_1} \LinOpInv{\alpha_1}{\beta_1} \bm{e}_1,
\end{equation} 
with shifts $\varrho_i = \mu_i / \nu_i$ and poles $\xi_i = \alpha_i / \beta_i$. 
The following procedure can be used to compute $\bm{x}$,
\begin{equation}
\label{eq:proc_multishift}
\begin{split}
& \bm{x} \leftarrow \bm{e}_1 \\
& \text{for $i =1,\hdots,m$} \\
& \; \begin{sqcases}
\bm{x} \leftarrow \gamma_i  \LinOp{\mu_i}{\nu_i} \LinOpInv{\alpha_i}{\beta_i} \bm{x}
\end{sqcases}
\end{split}.
\end{equation}
Here the $\gamma_i$ can be any suitable scaling factors. 

\begin{lemma}
\label{lemma:multishift_vec}
The vector $\bm{x}$ computed in equations \eqref{eq:vec_multishift} and \eqref{eq:proc_multishift} only has nonzero elements in its first $m{+}1$ entries.
\end{lemma}
\begin{proof}
The vector $\bm{x}$ is equal to:
\begin{equation*}
\begin{split}
\bm{x} = 
& \gamma \, \LinOpM{AB^{-1}}{\mu_m}{\nu_m} \LinOpMInv{AB^{-1}}{\alpha_m}{\beta_m} \hdots \\
& \qquad \qquad \LinOpM{AB^{-1}}{\mu_1}{\nu_1} \LinOpMInv{AB^{-1}}{\alpha_1}{\beta_1} \bm{e}_1 \\
= & \gamma \, q_{\Xi_{2,1:m}}(AB^{-1})^{-1} \, p(AB^{-1}) \bm{e}_1,
\end{split}
\end{equation*}
with $\Xi_{2,1:m}$ as defined in \cref{corr:rathess_qrpd} and $p$ a polynomial of degree $m$ with roots $\Rho$. Clearly, $\bm{x} \in \mathcal{Q}_{m+1}(AB^{-1},\bm{e}_1, \Xi_{2,1:m}) = \mathcal{E}_{m+1}$.
\end{proof}
%old proof
%\begin{proof}
%The proof is by induction on $m$.
%The case $m{=}1$ is covered by the discussion of \cref{ssec:introduce}.
%Denote $\bm{x}^{(j)}$ as the intermediate result after $j$ steps in the for loop of \eqref{eq:proc_multishift} are completed.
%Assume the lemma holds up to the case $m{-}1$, i.\ e.\ $\bm{x}^{(m{-}1)}$ only has nonzero elements in its first $m$ entries.
%In other words, $\bm{x}^{(m{-}1)} \in \mathcal{E}_m$, which is equivalent with $\bm{x}^{(m{-}1)} \in \mathcal{Q}_m(AB^{-1},\bm{e}_1,\Xi_{2,1:m{-}1})$ according to \cref{corr:rathess_qrpd}.
%Using properties of rational Krylov subspaces, there exists a polynomial $p$ of degree $m{-}1$ such that
%\begin{equation*}
%\bm{x}^{(m{-}1)} = q_{\Xi_{2,1:m{-}1}}(AB^{-1})^{-1} \, p(AB^{-1}) \, \bm{e}_1.
%\end{equation*}
%By construction $p$ has roots $\varrho_1, \hdots, \varrho_{m-1}$.
%From this it follows that
%\begin{equation*}
%\begin{split}
%\bm{x}^{(m)}
%& = \LinOp{\varrho_m}{} \LinOpInv{\xi_m}{} \, q_{\Xi_{2,1:m{-}1}}(AB^{-1})^{-1} \, p(AB^{-1}) \, \bm{e}_1 \\
%& = q_{\Xi_{2,1:m}}(AB^{-1})^{-1} \, \LinOp{\varrho_m}{} \, p(AB^{-1}) \, \bm{e}_1,
%\end{split}
%\end{equation*}
%such that $\bm{x}^{(m)} \in \mathcal{Q}_{m+1}(AB^{-1},\bm{e}_1,\Xi_{2,1:m}) = \mathcal{E}_{m+1}$.
%\end{proof}

\begin{remark}
No shifted systems $\LinOpInv{\alpha_i}{\beta_i} \bm{x}$ of full dimension $n$ need to be solved in order to compute $\bm{x}$ via the method in equation \eqref{eq:proc_multishift}.
At step $j$ of the loop, $\LinOp{\alpha_j}{\beta_j}$ has a zero in position $(j{+}1,j)$ and since $\bm{x} \in \mathcal{E}_j$, the system decouples and we essentially need to solve an $j{\times}j$ system in Hessenberg form.
The computational cost is $O(m^2)$, which is small as long as $m \ll n$.
\end{remark}

Given that $\bm{x} \in \mathcal{E}_{m+1}$, $m$ core transformations $C_1, \hdots, C_m$ can be computed such that
\begin{equation}
\label{eq:Qmultishift}
C_1^* \hdots C_m^* \bm{x} = Q^* \bm{x} = \alpha \bm{e}_1.
\end{equation}
The multishift step is initialized in the pair $(\hat{A},\hat{B}) = Q^* (A,B)$. The first $m{+}1$ rows in $(\hat{A},\hat{B})$ are affected by $Q^*$ and no longer are in Hessenberg form. 
They do have an interesting property:
%
\begin{theorem}
\label{thm:multishift}
Let $(A,B)$ be an $n{\times}n$ Hessenberg pair with poles $\Xi = \lbrace \xi_1, \hdots, \xi_{n-1} \rbrace$, $\Xi \cap \Lambda(A,B) = \varnothing$, and $A$, $B$ nonsingular matrices. Given $m{<}n$ shifts $\Rho_{1:m} = \lbrace \varrho_1, \hdots, \varrho_m \rbrace$, consider the transformation $Q$ computed according to equations \eqref{eq:vec_multishift} and \eqref{eq:Qmultishift}. The pair $(\hat{A},\hat{B}) = Q^* (A,B)$ has the property 
\begin{equation*}
\Lambda(\hat{A}_{2{:}m+1,1:m},\hat{B}_{2{:}m+1,1:m}) = \lbrace \varrho_1, \hdots, \varrho_m \rbrace.
\end{equation*}
\end{theorem}
%
\begin{proof}
From $(\hat{A},\hat{B}) = Q^* (A,B)$, it follows that $AB^{-1} Q \hat{B} = Q \hat{A}$. Furthermore, it follows from \cref{lemma:multishift_vec} and equation \eqref{eq:Qmultishift} that the first $m$ columns of this matrix relation satisfy
\begin{equation*}
AB^{-1} Q_{:,1:m+1}\hat{B}_{1:m+1,1:m} = Q_{:,1:m+1}\hat{A}_{1:m+1,1:m}.
\end{equation*}
Drawing from the results in \cite[Section 4.1]{Berljafa2015}, this is a \emph{generalized rational Krylov decomposition} of order $m{+}1$. 
All that is left to show, is that $Q_{:,1:m+1}$ spans the subspace $\mathcal{Q}_{m+1}(AB^{-1},\bm{q}_1,\Rho_{1:m})$. 
Accordingly, the eigenvalues of the lower $m{\times}m$ block of $(\hat{A}_{1:m+1,1:m},\hat{B}_{1:m+1,1:m})$ are equal to $\Rho_{1:m}$ based on the results in  \cite[Section 4.1]{Berljafa2015}.
The first $m{+}1$ columns indeed span the desired subspace:
\begin{align*}
\mathcal{R}(Q_{:,1:m+1}) 
& =  Q \, \mathcal{E}_{m+1} 
=  \mathcal{E}_{m+1}
=  \mathcal{Q}_{m+1}(AB^{-1},\bm{e}_1,\Xi_{2,1:m}) \\
& =  \mathcal{K}_{m+1}(AB^{-1}, q_{\Xi_{2,1:m}}(AB^{-1})^{-1}\bm{e}_1) \\
& =  \mathcal{K}_{m+1}(AB^{-1}, q_{\Rho_{1:m}}(AB^{-1})^{-1}\bm{q}_1)
=  \mathcal{Q}_{m+1}(AB^{-1},\bm{q}_1,\Rho_{1:m}).
\end{align*}
\end{proof}

In the second equality above we used the characteristic that $Q = C_m \hdots C_1$ does not change the span of the subspace $\mathcal{E}_{m+1}$.
In this step we loose the \emph{nestedness} property: the first $l \leq m$ columns of $Q$  do not span $\mathcal{Q}_l(AB^{-1},\bm{q}_1,\Rho_{1:l{-1}})$. 
The nestedness is also not prevalent in the first $m$ columns of $(\hat{A},\hat{B})$ since the upper Hessenberg structure is disturbed.




\subsection{Swapping poles and shifts}
XXXXXXX
The operation shown in \cref{fig:swap} swaps two single poles by acting on a $2{\times}2$ block. 
The mathematical description of the swapping operation is independent of the size the blocks.
The description is therefore kept general in terms of the blocksize.
Consider a matrix pair $(\hat{A},\hat{B})$, extracted from a Hessenberg pair $(A,B)$, that can be block partitioned as
%
\begin{align*}
\hat{A} = 
\begin{bmatrix}
\hat{A}_{11} & \hat{A}_{12} \\
0 & \hat{A}_{22}
\end{bmatrix}, \quad
\hat{B} = 
\begin{bmatrix}
\hat{B}_{11} & \hat{B}_{12} \\
0 & \hat{B}_{22}
\end{bmatrix},
\end{align*}
%
with $(\hat{A}_{11}, \hat{B}_{11})$ of size $n_1{\times}n_1$ and $(\hat{A}_{22}, \hat{B}_{22})$ of size $n_2{\times}n_2$.
In case of \cref{fig:swap} $n_1 = n_2 = 1$, but for the multishift setting $n_1=k$ with $k$ the degree of the implicit step.
The pair $(\hat{A},\hat{B})$ is always extracted in such a manner that the subdiagonal elements of $(A,B)$ are on the diagonal of $(\hat{A},\hat{B})$.

This problem is equivalent to the problem of reordering eigenvalues in the generalized
Schur form and the same techniques as introduced by K\aa gstr\"om \& Poromaa (1996)
\cite{Kagstrom1996} can be used. We shortly review the method for reordering the
eigenvalues, which, in our case, are poles in a Hessenberg pair. We assume that the
eigenvalues of $(\hat{A}_{11}, \hat{B}_{11})$ and $(\hat{A}_{22}, \hat{B}_{22})$ are
distinct, as otherwise no swap is required.
%and available in LAPACK \cite{Anderson1999} as \texttt{xTGEX2} and \texttt{xTGEXC}

The problem is to find unitary $Q$ and $Z$ matrices of size $n_1 + n_2$ such that,
%
\begin{align*}
(\check{A}, \check{B}) = Q^* (\hat{A}, \hat{B}) Z =
\left(
\begin{bmatrix}
\check{A}_{22} & \check{A}_{12} \\
0 & \check{A}_{11}
\end{bmatrix}
,
\begin{bmatrix}
\check{B}_{22} & \check{B}_{12} \\
0 & \check{B}_{11}
\end{bmatrix}
\right),
\end{align*}
with $\Lambda(\hat{A}_{11},\hat{B}_{11}) = \Lambda(\check{A}_{11},\check{B}_{11})$, $\Lambda(\hat{A}_{22},\hat{B}_{22}) = \Lambda(\check{A}_{22},\check{B}_{22})$. To this end, consider,
%
\begin{align*}
L = 
\begin{bmatrix}
 & I \\
I & Y 
\end{bmatrix},
\qquad
R =
\begin{bmatrix}
X & I \\
I & \\
\end{bmatrix},
\end{align*}
and multiply $(\hat{A},\hat{B})$ from left with $L$ and right with $R$ to get
%
\begin{align*}
L (\hat{A},\hat{B}) R =
\left(
\begin{bmatrix}
\hat{A}_{22} & \\
\hat{A}_{12} + \hat{A}_{11} X + Y \hat{A}_{22} & \hat{A}_{11}
\end{bmatrix}
,
\begin{bmatrix}
\hat{B}_{22} & \\
\hat{B}_{12} + \hat{B}_{11} X + Y \hat{B}_{22} & \hat{B}_{11}
\end{bmatrix}
\right).
\end{align*}
It is immediate that $L$ and $R$ achieve the desired swapping if
\begin{eqnarray}
\label{eq:genSylv}
%\begin{split}
\hat{A}_{11} X + Y \hat{A}_{22} = - \hat{A}_{12} \\
\nonumber \hat{B}_{11} X + Y \hat{B}_{22} = - \hat{B}_{12}.
%\end{split}
\end{eqnarray}
This is a \emph{generalized Sylvester equation} which can be solved from the $2 n_1 n_2{\times}2 n_1 n_2$ system $M x = b$ obtained from the vectorization of \cref{eq:genSylv}:
%
\begin{align*}
M =
\begin{bmatrix}
I_{n_2} \otimes \hat{A}_{11} & - \hat{A}_{22}^T \otimes I_{n_1} \\
I_{n_2} \otimes \hat{B}_{11} & - \hat{B}_{22}^T \otimes I_{n_1}
\end{bmatrix},
\quad
x =
\begin{bmatrix}
\text{vec}(X) \\
\text{vec}(Y)
\end{bmatrix},
\quad
b =
\begin{bmatrix}
-\text{vec}(\hat{A}_{12}) \\
-\text{vec}(\hat{B}_{12})
\end{bmatrix}.
\end{align*}
The solution gives us $L$ and $R$ which are not unitary and can be ill conditioned. To overcome this, the decompositions $L = RQ^*$, $R = ZS$ are made; respectively an $RQ$ and a $QR$ decomposition. The matrices $Q$ and $Z$ are unitary matrices that perform the swapping operation.
Further details are found available in \cite{Kagstrom1996}.

XXXXX


\subsubsection*{Swapping.}
After the $m$ shifts are initialized, they can be swapped with respectively $\xi_{m+1}, \hdots, \xi_{n-1}$ via the procedure discussed in \cref{ssec:swap} with $n_1 = m$, $n_2 = 1$ until they arrive at position $n{-}m{+}1{:}n,n{-}m{:}n{-}1$ of $(A,B)$. 
To compute the transformations for a single swap, a $2m{\times}2m$ system needs to be solved, which comes at a computational complexity of $O(8m^3)$.
The first swap is illustrated in \cref{fig:multishift_1} below.

\begin{figure}[htp]
\label{fig:multishift_1}
\centering
\input{../fig/fig_multishift.tikz}
\caption{First swap in the multishift step with $m{=}4$ shifts. The light gray area covers the Hessenberg part of the matrix pair, the dark gray area is the part of the pair which is disturbed by the introduction of the shifts.
The magnified areas show the $4{\times}4$ block in the darker shaded region and the multishift block together with the next pole $\oplus{/}\ominus$ in the lighter shaded region.
The dotted sections in the matrix pair are the rows and columns which are affected during the execution of the swap.}
\end{figure}

\subsubsection*{Finalization.}
At the end of the multishift RQZ step, we have the opportunity to introduce $m$ new poles $\hat{\xi}_{n-m} \hdots \hat{\xi}_{n-1}$.
This can be achieved in two steps.
First, the subdiagonal block at position $n{-}m{+}1{:}n, n{-}m{:}n{-}1$ of $A$ and $B$ is to be transformed to generalized Schur form. 
This restores the matrix pair to Hessenberg form. 
By \cref{thm:multishift}, and ignoring the effects of \emph{shift blurring}, we know that after this transformation the last $m$ poles are equal to$\varrho_1, \hdots, \varrho_m$.
The order in which these appear on the subdiagonal depends on the reduction to generalized Schur form, but they can obviously be reordered.
In a second phase, the $m$ shifts can be replaced by any set of $m$ new poles employing the following procedure:
\begin{equation}\label{eq:updatepolesmultishift}
\begin{split}
& \text{for $i =m,\hdots,1$} \\
& \; \begin{sqcases}
\xi_{n-1} \leftarrow \hat{\xi}_{n-i} \\
\text{for $j = i-1,\hdots,1$} \\
\quad \begin{sqcases}
\text{\texttt{swap}}(\xi_{i-1},\xi_{i})
\end{sqcases}
\end{sqcases},
\end{split}
\end{equation}
where we used the condensed notation $\xi_{n-1} \leftarrow \hat{\xi}_{n-i}$ for the procedure from \cref{ssec:introduce} to introduce a new last pole in the Hessenberg pair. This method updates the pole set of the Hessenberg pair to $\lbrace \xi_{m+1}$, $\hdots$ , $\xi_{n-1}$, $\hat{\xi}_{n-m}$, $\hdots$ , $\hat{\xi}_{n-1} \rbrace$.
This finalizes the multishift RQZ step.
%
\subsubsection*{Decoupled multishifts.}
The multishift procedure discussed thus far can be seen as a generalization of the multishift step in the QZ method \cite{Kagstrom2007}.
The $m$ shifts are coupled together in an $m{\times}m$ subdiagonal block. 
Decoupling them can be achieved in two ways. 
A first possibility is to restore the Hessenberg form  after the introduction of the $m{\times}m$ multishift block by reducing the block to generalized Schur form.
A second possibility is to introduce the $m$ shift seperately via a procedure equivalent with equation \eqref{eq:updatepolesmultishift}: introduce shift $\varrho_m$ as the first pole, swap it to position $(m{+}1,m)$, introduce $\varrho_{m-1}$, swap it to position $(m,m{-}1)$, etc.

With decoupled shifts, the next pole $\xi_{m+1}$ can be swapped through every shift individually in order the shift the $m{\times}m$ block one row done and one column to the right in its entirety.
This process is illustrated in \cref{fig:multishift_2}.
Note that in order to shift the entire block a total of $m$ swaps are required. These can be computed based on the shaded area in the magnification in \cref{fig:multishift_2}.
This comes down to solving $m$ systems of size $2{\times}2$ at a total computational complexity of $O(8m)$.
The transformations can be accumulated such that the dotted areas of the matrix pair can be updated  with the same efficiency as in \cref{fig:multishift_1}.

The advantage of a decoupled multishift step is twofold. First, the computation of the transformations requires less operations. Second, the effect of shift blurring can be carefully monitored and is expected to be less severe.
Shift blurring \cite{Kagstrom2007} is the effect that for increasing $m$, the shifts in the subdiagonal block can be severely affected by roundoff errors during the implicit step. 

\begin{figure}[htp]
\label{fig:multishift_2}
\centering
\input{../fig/fig_multishift_2.tikz}
\caption{First swap in the multishift step with $m=4$ decoupled shifts. The light gray area covers the Hessenberg part of the matrix pair The magnified portions show the $4$ shifts $\odot{/}\oslash$ and indicate how they can be swapped with the next pole $\oplus{/}\ominus$ by four $2{\times}2$ swaps by only using the shaded part of the matrix pair. The dotted sections in the matrix pair are the rows and columns which are affected during the execution of the swap.}
\end{figure}


\subsection{Numerical experiment.}


%% CONVERGENCE DISCUSSION FOR THE MULTISHIFT CASE
\subsubsection{Convergence.}
The convergence theory of \cref{ssec:subspaceiter} can be generalized to the multishift setting to show that it also implements subspace iteration with a change of basis driven by rational functions that are a concatenation of the elementary rational functions in \cref{thm:rational_subspace_it}. 
More precisely, if the Hessenberg pair $(A,B)$ with poles $\Xi = \lbrace \xi_1, \hdots, \xi_{n-1} \rbrace$ is updated to a pair $(\hat{A}, \hat{B}) = Q^* (A,B) Z$ with poles $\hat{\Xi} = \lbrace \xi_{m+1}, \hdots, \xi_{n-1}, \hat{\xi}_{n-m}, \hdots, \hat{\xi}_{n-1} \rbrace$ with $\bm{q}_1 = p_{\Rho_{1:m}}(AB^{-1}) \, q_{\Xi_{1:m}}(AB^{-1})^{-1} \bm{e}_1$ and $m < k < n$. Then,

\begin{equation}
\begin{split}
\mathcal{R}(Q_{:,1:k}) = \, & f_{Q_{:,1:k}}(AB^{-1}) \, \mathcal{E}_k \\
\text{with} \quad & f_{Q_{:,1:k}}(z) = p_{\Rho_{1:m}}(z) \, q_{\Xi_{k:m+k-1}}(z)^{-1}\\
\mathcal{R}(Z_{:,1:k}) = \, & f_{Z_{:,1:k}}(B^{-1}A) \, \mathcal{E}_k \\
\text{with} \quad & f_{Z_{:,1:k}}(z) = p_{\Rho_{1:m}}(z) \, q_{\Xi_{k+1:m+k}}(z)^{-1}.
\end{split}
\end{equation}


==> tab/tab_numexp1.tex <==
\begin{tabular}{l | l | l | l}
Matrix & condition & $\Gamma_{1}$ & $\Gamma_{2,3}$ \\ \hline
%
$A$: MHD416A&  $2.4 \cdot 10^{25}$ & \multirow{2}{*}{$e(-1.3,1.5,3,0)$} & \multirow{2}{*}{$e(-0.6{\pm}105i,0.65,98,\pm0.005)$} \\
%
$B$: MHD416B & $5.1 \cdot 10^{9}$  & & \\ \hline
%
$A$: MHD1280A & $1.0 \cdot 10^{25}$ & \multirow{2}{*}{$e(-25,27,6,0)$} & \multirow{2}{*}{$e(-10{\pm}280i,6,270,\pm0.05)$}\\
%
$B$: MHD1280B & $6.0 \cdot 10^{12}$ & &
\end{tabular}


==> tab/tab_numexp2b.tex <==
% total iterations
%\begin{tabular}{l | l | l | l | l | l | l | l | l |}
% & \multicolumn{4}{|c|}{\emph{Cavity flow}} & \multicolumn{4}{|c|}{\emph{Obstacle flow}} \\ 
%$\Xi$ & error $A$ & error $B$ & iter & $\%$ & error $A$ & error $B$ & iter & $\%$ \\ \hline
%$\infty$ & $7.45 \cdot 10^{-15}$ & $4.35 \cdot 10^{-15}$ & $5609$ & $100$ & $9.24 \cdot 10^{-15}$ & $7.81 \cdot 10^{-15}$ & $6141$ & $100$ \\
%W & $7.82 \cdot 10^{-15}$ & $4.14 \cdot 10^{-15}$ & $5248$ & $93.6$ & $8.76 \cdot 10^{-15}$ & $7.83 \cdot 10^{-15}$ & $5591$ & $91.0$ \\
%$\Gamma_1$ & $7.77 \cdot 10^{-15}$ & $4.28 \cdot 10^{-15}$ & $5583$ & $99.5$ & $9.22 \cdot 10^{-15}$ & $8.06 \cdot 10^{-15}$ & $6103$ & $99.4$\\
%$\Gamma_2$ & $7.72 \cdot 10^{-15}$ & $4.32 \cdot 10^{-15}$ & $5575$ & $99.4$ & $9.19 \cdot 10^{-15}$ & $8.06 \cdot 10^{-15}$ & $6033$ & $98.2$\\
%\end{tabular}

% iterations/ev
\begin{tabular}{l | l | l | l | l | l | l | l | l |}
 & \multicolumn{4}{|c|}{\emph{Cavity flow}} & \multicolumn{4}{|c|}{\emph{Obstacle flow}} \\ 
$\Xi$ & error $A$ & error $B$ & it/ev & $\%$ & error $A$ & error $B$ & it/ev & $\%$ \\ \hline
%
$\infty$ & $7.5 \cdot 10^{-15}$ & $4.4 \cdot 10^{-15}$ & $2.27$ & $100$ & $9.2 \cdot 10^{-15}$ & $7.8 \cdot 10^{-15}$ & $2.47$ & $100$ \\
%
Wilk. & $7.8 \cdot 10^{-15}$ & $4.1 \cdot 10^{-15}$ & $2.13$ & $93.6$ & $8.8 \cdot 10^{-15}$ & $7.8 \cdot 10^{-15}$ & $2.25$ & $91.0$ \\
% %
% $\Gamma_1$ & $7.8 \cdot 10^{-15}$ & $4.3 \cdot 10^{-15}$ & $2.26$ & $99.5$ & $9.2 \cdot 10^{-15}$ & $8.1 \cdot 10^{-15}$ & $2.45$ & $99.4$\\
% %
% $\Gamma_2$ & $7.7 \cdot 10^{-15}$ & $4.3 \cdot 10^{-15}$ & $2.26 $ & $99.4$ & $9.2 \cdot 10^{-15}$ & $8.1 \cdot 10^{-15}$ & $2.42$ & $98.2$\\
% %
\end{tabular}

